Encryption-Friendly LLM Architecture

Large language models (LLMs) offer personalized responses based on user interactions, but this use case raises serious privacy concerns. Homomorphic encryption (HE) is a cryptographic protocol supporting arithmetic computations in encrypted states and provides a potential solution for privacy-preserving machine learning (PPML). However, the computational intensity of transformers poses challenges for applying HE to LLMs. In this work, we propose a modified HE-friendly transformer architecture with an emphasis on inference following personalized (private) fine-tuning. Utilizing LoRA fine-tuning and Gaussian kernels, we achieve significant computational speedups -- 6.94x for fine-tuning and 2.3x for inference -- while maintaining performance comparable to plaintext models. Our findings provide a viable proof of concept for offering privacy-preserving LLM services in areas where data protection is crucial. Our code is available on GitHub.

==> codes/docs/acb40c4a-f477-494b-aefa-dddf54f6f382 <==
{"id":"r0.133682665371176","lines":[{"id":"n0.6271239224103194","blocks":[]},{"id":"n0.1584590619804962","blocks":[{"id":"n0.521132095910138","text":"\\diagram","type":"composite","elements":{"de5271171352809016":{"id":"de5271171352809016","lines":[{"id":"n0.4013356768360721","blocks":[{"id":"n0.9128069386535047","text":"rank","style":{"fontSize":"\\footnotesize"}}]}],"shape":{"data":{"p":{"x":0.33333333333331794,"y":61.666666666666686}},"anchor":"left-top"},"isTextMode":true},"de05193635176158562":{"id":"de05193635176158562","lines":[{"blocks":[{"id":"n0.029356877370279255","text":"128","style":{"fontSize":"\\footnotesize"}}],"id":"n0.6857617914911578"}],"shape":{"data":{"p":{"x":46.66666666666667,"y":44.333333333333336}},"anchor":"left-top"},"isTextMode":true},"de3021048323491804":{"id":"de3021048323491804","lines":[{"blocks":[{"text":"rank","style":{"fontSize":"\\footnotesize"},"id":"n0.7856401960961072"}],"id":"n0.5282393349598229"}],"shape":{"data":{"p":{"x":26.333333333333314,"y":210.66666666666669}},"anchor":"left-top"},"isTextMode":true},"de3540698230350725":{"id":"de3540698230350725","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.909627645056069"}],"id":"n0.5817272361195118"}],"shape":{"data":{"p":{"x":73.33333333333331,"y":193.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de6178331023929506":{"id":"de6178331023929506","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.9789193672514063"}],"id":"n0.8130619373764332"}],"shape":{"data":{"p":{"x":106.66666666666666,"y":44.666666666666664}},"anchor":"left-top"},"isTextMode":true},"de3254922127718054":{"id":"de3254922127718054","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.0963483255805706"}],"id":"n0.8731050371553959"}],"shape":{"data":{"p":{"x":287,"y":44.66666666666667}},"anchor":"left-top"},"isTextMode":true},"de846230227270492":{"id":"de846230227270492","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.2990946039400577"}],"id":"n0.20194181219475738"}],"shape":{"data":{"p":{"x":24.333333333333314,"y":234.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de43406213075574573":{"id":"de43406213075574573","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.9639586597597096"}],"id":"n0.5384658896250307"}],"shape":{"data":{"p":{"x":276.3333333333333,"y":147.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de7082527372726444":{"id":"de7082527372726444","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.9763240019719925"}],"id":"n0.8723445575400424"}],"shape":{"data":{"p":{"x":228.33333333333331,"y":187.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de13836529581489088":{"id":"de13836529581489088","lines":[{"id":"n0.12274929055410722","blocks":[{"id":"n0.279286342574643","text":"a"}]}],"shape":{"data":{"p":{"x":54,"y":65}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de6510870482652797":{"id":"de6510870482652797","lines":[{"blocks":[{"id":"n0.7929456055184831","text":"b"}],"id":"n0.5600375748146931"}],"shape":{"data":{"p":{"x":114,"y":66}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de27206745070898997":{"id":"de27206745070898997","lines":[{"blocks":[{"id":"n0.9548072542726482","text":"f"}],"id":"n0.036105015636802795"}],"shape":{"data":{"p":{"x":293,"y":64}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de3637281806726733":{"id":"de3637281806726733","lines":[{"blocks":[{"text":"a","id":"n0.281474309644002"}],"id":"n0.20844189439422411"}],"shape":{"data":{"p":{"x":82,"y":214}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de1190302592879302":{"id":"de1190302592879302","lines":[{"blocks":[{"text":"b","id":"n0.34013290559749465"}],"id":"n0.39883501699082813"}],"shape":{"data":{"p":{"x":140,"y":215}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de6433898381197358":{"id":"de6433898381197358","lines":[{"blocks":[{"id":"n0.5783781059571189","text":"c"}],"id":"n0.35384865034885715"}],"shape":{"data":{"p":{"x":81,"y":228}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de23691462518175088":{"id":"de23691462518175088","lines":[{"blocks":[{"id":"n0.26549063102607673","text":"d"}],"id":"n0.451659542752604"}],"shape":{"data":{"p":{"x":139,"y":229}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de6697213339170929":{"id":"de6697213339170929","lines":[{"blocks":[{"id":"n0.2947226719817335","text":"e"}],"id":"n0.4795804504420511"}],"shape":{"data":{"p":{"x":81,"y":242}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de7202959532078801":{"id":"de7202959532078801","lines":[{"blocks":[{"id":"n0.6835362805393077","text":"f"}],"id":"n0.4616071493267835"}],"shape":{"data":{"p":{"x":139,"y":243}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de5833350304434612":{"id":"de5833350304434612","lines":[{"blocks":[{"text":"a","id":"n0.233101515217367"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.8948057867263983"}],"id":"n0.22536645859665905"}],"id":"n0.24361883243139215"}},"id":"n0.4574831057922897"}],"id":"n0.912810641858901"}],"shape":{"data":{"p":{"x":285,"y":175.33333333333334}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de7880597539196552":{"id":"de7880597539196552","lines":[{"blocks":[{"id":"n0.13428124196921454","text":"b"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.0063776509229067635"}],"id":"n0.8482322921803847"}],"id":"n0.7265404916740146"}},"id":"n0.45948131505792844"}],"id":"n0.03068603412955051"}],"shape":{"data":{"p":{"x":346,"y":175.66666666666669}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de6482563091284139":{"id":"de6482563091284139","lines":[{"blocks":[{"id":"n0.5208748767118185","text":"e"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.1543869892405556"}],"id":"n0.9688577164385499"}],"id":"n0.2776540036262689"}},"id":"n0.0513652004823828"}],"id":"n0.5007669102533678"}],"shape":{"data":{"p":{"x":281.33333333333337,"y":285.33333333333337}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de7901576719656223":{"id":"de7901576719656223","lines":[{"blocks":[{"text":"f","id":"n0.7972568171744325"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.5142223046491208"}],"id":"n0.9771093816082077"}],"id":"n0.8597677525217777"}},"id":"n0.9770476504577239"}],"id":"n0.7802027865460996"}],"shape":{"data":{"p":{"x":341.66666666666674,"y":286.33333333333337}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de6606157978055531":{"id":"de6606157978055531","lines":[{"blocks":[{"id":"n0.9219287598410861","text":"e"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.025615132330217838","text":"r"}],"id":"n0.01464525524766902"}],"id":"n0.053375853493953906"}},"id":"n0.13883586079516852"}],"id":"n0.22945900809923803"}],"shape":{"data":{"p":{"x":431.00000000000006,"y":286.6666666666667}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de9329668029063163":{"id":"de9329668029063163","lines":[{"blocks":[{"text":"f","id":"n0.18889291719661983"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4572013987454162","text":"r"}],"id":"n0.01617697407713936"}],"id":"n0.5882601486010204"}},"id":"n0.8161196066905299"}],"id":"n0.5569892442451241"}],"shape":{"data":{"p":{"x":491.0000000000001,"y":286.6666666666667}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de19841006597672717":{"id":"de19841006597672717","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.4474442083461059"}],"id":"n0.015748287197899558"}],"shape":{"data":{"p":{"x":336.66666666666663,"y":146.66666666666669}},"anchor":"left-top"},"isTextMode":true},"de07552938624330774":{"id":"de07552938624330774","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.9890200449698974"}],"id":"n0.5293439546847958"}],"shape":{"data":{"p":{"x":487,"y":146.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de6543214542300515":{"id":"de6543214542300515","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.3816101744577298"}],"id":"n0.9113533128916058"}],"shape":{"data":{"p":{"x":426.3333333333333,"y":145.66666666666669}},"anchor":"left-top"},"isTextMode":true},"de7574238055940739":{"id":"de7574238055940739","lines":[{"blocks":[{"id":"n0.9107091993368355","text":"a"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"r","id":"n0.7140650105520507"}],"id":"n0.20312339232869836"}],"id":"n0.07593281113625716"}},"id":"n0.723499969625647"}],"id":"n0.8916209140592821"}],"shape":{"data":{"p":{"x":431.33333333333337,"y":190.33333333333334}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de7099591514403822":{"id":"de7099591514403822","lines":[{"blocks":[{"id":"n0.4702660652900057","text":"b"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.029129947365508446","text":"r"}],"id":"n0.46894275651486006"}],"id":"n0.238108179421199"}},"id":"n0.8313939467004845"}],"id":"n0.4382082993676488"}],"shape":{"data":{"p":{"x":491.3333333333335,"y":190}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de6905962216097146":{"id":"de6905962216097146","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.7731410549422975"}],"id":"n0.5327355769595381"}],"shape":{"data":{"p":{"x":532.6666666666666,"y":183.66666666666669}},"anchor":"left-top"},"isTextMode":true},"de6634382220376858":{"id":"de6634382220376858","lines":[{"blocks":[{"id":"n0.586023349931055","text":"ct"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"11","id":"n0.9653714146290966"}],"id":"n0.4734590711634452"}],"id":"n0.3248261051221777"}},"id":"n0.9840013166146373"}],"id":"n0.49793118114329227"}],"shape":{"data":{"p":{"x":311.6666666666667,"y":229.99999999999997}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de11857513190146118":{"id":"de11857513190146118","lines":[{"blocks":[{"text":"ct","id":"n0.5648653365257932"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1r","id":"n0.5113126728297825"}],"id":"n0.004749653626144434"}],"id":"n0.43821179307408076"}},"id":"n0.4726939917157964"}],"id":"n0.17007431484117053"}],"shape":{"data":{"p":{"x":460.3333333333333,"y":229.66666666666663}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de3977587621824119":{"id":"de3977587621824119","lines":[{"blocks":[{"text":"ct","id":"n0.2938962836222907"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"31","id":"n0.4317026842914824"}],"id":"n0.6574725028389363"}],"id":"n0.3287014453411208"}},"id":"n0.32519773223823223"}],"id":"n0.38746791859367957"}],"shape":{"data":{"p":{"x":311.33333333333337,"y":322.66666666666663}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de4790639906884946":{"id":"de4790639906884946","lines":[{"blocks":[{"text":"ct","id":"n0.9347070009097664"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"3r","id":"n0.8108249958240477"}],"id":"n0.2406257479135907"}],"id":"n0.44846349990510403"}},"id":"n0.3099229125384759"}],"id":"n0.2018694373292209"}],"shape":{"data":{"p":{"x":460.33333333333337,"y":324.3333333333333}},"anchor":"left-top","settings":{"fontSize":{"value":0.5882}}},"isMathDisplayMode":true},"de345712966734397":{"id":"de345712966734397","lines":[{"id":"n0.636797397764653","blocks":[{"id":"n0.18540868319421855","text":"⋯"}]}],"shape":{"data":{"p":{"x":382,"y":187.00000000000003}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de9325712331975726":{"id":"de9325712331975726","lines":[{"blocks":[{"text":"⋯","id":"n0.5533280874267159"}],"id":"n0.8866149785471449"}],"shape":{"data":{"p":{"x":381.6666666666667,"y":285}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de3589645524095135":{"id":"de3589645524095135","lines":[{"blocks":[{"text":"⋯","id":"n0.905289066141397"}],"id":"n0.33847917249038884"}],"shape":{"data":{"p":{"x":329.85782055924534,"y":237.2429460093379},"rotation":89.42},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de7511499864209452":{"id":"de7511499864209452","lines":[{"blocks":[{"text":"⋯","id":"n0.30152298710539127"}],"id":"n0.2673804757018765"}],"shape":{"data":{"p":{"x":479.524487225912,"y":236.57627934267126},"rotation":89.42},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de8765002708313898":{"id":"de8765002708313898","lines":[{"blocks":[{"text":"rank","style":{"fontSize":"\\footnotesize"},"id":"n0.47552312050595824"}],"id":"n0.2964872782851007"}],"shape":{"data":{"p":{"x":376.3333333333333,"y":40.666666666666686}},"anchor":"left-top"},"isTextMode":true},"de01608433901004558":{"id":"de01608433901004558","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.6824026838523665"}],"id":"n0.26932998078311154"}],"shape":{"data":{"p":{"x":423.3333333333333,"y":23.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de3021726648321661":{"id":"de3021726648321661","lines":[{"blocks":[{"text":"128","style":{"fontSize":"\\footnotesize"},"id":"n0.5316166143662537"}],"id":"n0.4164856255308862"}],"shape":{"data":{"p":{"x":374.3333333333333,"y":64.33333333333337}},"anchor":"left-top"},"isTextMode":true},"de7985812661804197":{"id":"de7985812661804197","lines":[{"blocks":[{"text":"a","id":"n0.888526440570351"}],"id":"n0.6035727352924569"}],"shape":{"data":{"p":{"x":432,"y":44}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de159711201599688":{"id":"de159711201599688","lines":[{"blocks":[{"text":"b","id":"n0.44487369437187074"}],"id":"n0.24272153771387783"}],"shape":{"data":{"p":{"x":490,"y":45}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de4617499796300588":{"id":"de4617499796300588","lines":[{"blocks":[{"text":"c","id":"n0.2865697176262383"}],"id":"n0.241645728532778"}],"shape":{"data":{"p":{"x":431,"y":58}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de8219317853178871":{"id":"de8219317853178871","lines":[{"blocks":[{"text":"d","id":"n0.4786872929174051"}],"id":"n0.48910549021293037"}],"shape":{"data":{"p":{"x":489,"y":59}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de5008797815077799":{"id":"de5008797815077799","lines":[{"blocks":[{"text":"e","id":"n0.44875829916524346"}],"id":"n0.7072332775477157"}],"shape":{"data":{"p":{"x":431,"y":72}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de8090017574307025":{"id":"de8090017574307025","lines":[{"blocks":[{"text":"f","id":"n0.10960028873944294"}],"id":"n0.826156673248382"}],"shape":{"data":{"p":{"x":489,"y":73}},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isMathDisplayMode":true},"de2935203224337839":{"id":"de2935203224337839","lines":[{"blocks":[{"text":"b","id":"n0.7385682360501831"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.7444007553427598"}],"id":"n0.4569517085955537"}],"id":"n0.6257626313497029"}},"id":"n0.42943196780921045"}],"id":"n0.7891153222855136"}],"shape":{"data":{"p":{"x":345.6666666666667,"y":168.33333333333334}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de8108944425854294":{"id":"de8108944425854294","lines":[{"blocks":[{"text":"b","id":"n0.12754267204432512"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.31336632284594246"}],"id":"n0.43006970348885765"}],"id":"n0.20356262207038722"}},"id":"n0.648420893246906"}],"id":"n0.9656345184991717"}],"shape":{"data":{"p":{"x":345.33333333333337,"y":219.33333333333334}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de42924149977042503":{"id":"de42924149977042503","lines":[{"blocks":[{"text":"b","id":"n0.6869581539406955"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.6291148605536792"}],"id":"n0.07693913837302602"}],"id":"n0.0863741210835618"}},"id":"n0.3578269343601552"}],"id":"n0.06141149811109381"}],"shape":{"data":{"p":{"x":345.00000000000006,"y":212}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de4133733128847432":{"id":"de4133733128847432","lines":[{"blocks":[{"text":"a","id":"n0.993573853201208"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.044361947494450105"}],"id":"n0.6057137813689555"}],"id":"n0.9672635085109942"}},"id":"n0.5181153479052096"}],"id":"n0.40952897918617204"}],"shape":{"data":{"p":{"x":286,"y":218.66666666666669}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de8538801245695513":{"id":"de8538801245695513","lines":[{"blocks":[{"text":"a","id":"n0.9529491942121682"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.351992930477667"}],"id":"n0.5559981747631841"}],"id":"n0.2747190678970184"}},"id":"n0.8270681379897371"}],"id":"n0.0921714565890479"}],"shape":{"data":{"p":{"x":285.3333333333333,"y":211.33333333333337}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de7671145984065686":{"id":"de7671145984065686","lines":[{"blocks":[{"text":"a","id":"n0.8583517871589676"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.5669916506879014"}],"id":"n0.5026106138662325"}],"id":"n0.938233599876757"}},"id":"n0.417032987487544"}],"id":"n0.025808062355950012"}],"shape":{"data":{"p":{"x":284.6666666666667,"y":167.33333333333334}},"anchor":"left-top","settings":{"fontSize":{"value":0.4118}}},"isMathDisplayMode":true},"de5051579701774151":{"id":"de5051579701774151","lines":[{"id":"n0.11493028185995002","blocks":[{"id":"n0.04461023161771327","text":"(a) LoRA-friendly packing"}]}],"shape":{"data":{"p":{"x":14,"y":5}},"anchor":"left-top"},"isTextMode":true},"de42610462356144585":{"id":"de42610462356144585","lines":[{"blocks":[{"text":"(b) Split & repeat row-wise","id":"n0.030137959352703803"}],"id":"n0.803912946025368"}],"shape":{"data":{"p":{"x":15,"y":135}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di3109559571301146","items":[],"style":{}},"shapes":[{"id":"dp4228447632390584","type":"rectangle","data":{"p1":{"x":30.5,"y":68.5},"p2":{"x":90.96023559570312,"y":82.8}},"style":{"fillColor":"none"}},{"id":"dp5188270355547413","type":"rectangle","data":{"p1":{"x":90.96023559570312,"y":68.5},"p2":{"x":151.42047119140625,"y":82.8}},"style":{"fillColor":"none"}},{"id":"dp20374191941973585","type":"rectangle","data":{"p1":{"x":151.42047119140625,"y":68.5},"p2":{"x":270.6,"y":82.8}}},{"id":"dp4462057041346257","type":"rectangle","data":{"p1":{"x":270.6,"y":68.5},"p2":{"x":331.06023559570315,"y":82.8}}},{"id":"dp2579824264084265","type":"rectangle","data":{"p1":{"x":57.03333333333333,"y":217.3},"p2":{"x":117.49356892903646,"y":231.60000000000002}}},{"id":"dp48041368525768524","type":"rectangle","data":{"p1":{"x":117.49356892903646,"y":217.3},"p2":{"x":177.95380452473958,"y":231.60000000000002}}},{"id":"dp5991912603338219","type":"rectangle","data":{"p1":{"x":57.03333333333333,"y":231.70000000000002},"p2":{"x":117.49356892903646,"y":246}}},{"id":"dp5782547455884233","type":"rectangle","data":{"p1":{"x":117.49356892903646,"y":231.70000000000002},"p2":{"x":177.95380452473958,"y":246}}},{"id":"dp8046310426598651","type":"rectangle","data":{"p1":{"x":57.03333333333333,"y":246},"p2":{"x":117.49356892903646,"y":260.3}}},{"id":"dp6309384147423494","type":"rectangle","data":{"p1":{"x":117.49356892903646,"y":246},"p2":{"x":177.95380452473958,"y":260.3}}},{"id":"dp09389474598757008","type":"rectangle","data":{"p1":{"x":57.03333333333333,"y":260.3},"p2":{"x":117.49356892903646,"y":276.5}},"style":{"fillColor":[218,216,216,0.6]}},{"id":"dp30787065938484925","type":"rectangle","data":{"p1":{"x":117.49356892903646,"y":260.3},"p2":{"x":177.95380452473958,"y":276.5}},"style":{"fillColor":[218,216,216,0.6]}},{"id":"da547896642682246","data":[{"p1":{"x":30.5,"y":68.5},"p2":{"x":30.5,"y":82.8},"cp":{"dx":-4.166666666666664,"dy":5.833333333333336},"cp2":{"dx":-4.166666666666664,"dy":-6.799999999999997}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da7994857226400138","data":[{"p1":{"x":30.5,"y":68.5},"p2":{"x":90.96023559570312,"y":68.5},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da36592948940259973","data":[{"p1":{"x":57.03333333333333,"y":217.40000000000003},"p2":{"x":57.03333333333333,"y":231.70000000000002},"cp":{"dx":-4.166666666666664,"dy":5.833333333333336},"cp2":{"dx":-4.166666666666664,"dy":-6.799999999999997}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da8206427081271903","data":[{"p1":{"x":57.03333333333333,"y":217.40000000000003},"p2":{"x":117.49356892903643,"y":217.40000000000003},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da732018465836888","data":[{"p1":{"x":90.49999999999999,"y":68.83333333333331},"p2":{"x":150.96023559570312,"y":68.83333333333331},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da6137574994059685","data":[{"p1":{"x":270.8333333333333,"y":68.83333333333333},"p2":{"x":331.29356892903644,"y":68.83333333333333},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da3811866905700785","data":[{"p1":{"x":57.03333333333333,"y":217.40000000000003},"p2":{"x":57.03333333333333,"y":276.5},"cp":{"dx":-10.033333333333331,"dy":25.09999999999998},"cp2":{"dx":-9.033333333333331,"dy":-18}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp12376304958365547","type":"down-arrow","data":{"p1":{"x":198.66666666666666,"y":230.33333333333331},"p2":{"x":221.5237833658854,"y":251.19047292073566},"rotation":269.56}},{"id":"dp054751518248259856","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":170.3},"p2":{"x":321.4935689290364,"y":177.5999984741211}}},{"id":"dp39348110210474774","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":177.5999984741211},"p2":{"x":321.4935689290364,"y":184.89999694824218}}},{"id":"dp44457172813970525","type":"rectangle","data":{"p1":{"x":321.4935689290364,"y":170.3},"p2":{"x":381.95380452473955,"y":177.5999984741211}}},{"id":"dp3127543282094525","type":"rectangle","data":{"p1":{"x":321.4935689290364,"y":177.5999984741211},"p2":{"x":381.95380452473955,"y":184.89999694824218}}},{"id":"dp931661174953754","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":214.09999084472645},"p2":{"x":321.4935689290364,"y":221.39998931884753}}},{"id":"dp5769943298469158","type":"rectangle","data":{"p1":{"x":321.4935689290364,"y":214.09999084472645},"p2":{"x":381.95380452473955,"y":221.39998931884753}}},{"id":"dp027923827816024316","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":221.39998931884753},"p2":{"x":321.4935689290364,"y":228.6999877929686}}},{"id":"dp06783360654080717","type":"rectangle","data":{"p1":{"x":321.4935689290364,"y":221.39998931884753},"p2":{"x":381.95380452473955,"y":228.6999877929686}}},{"id":"da8401248687083274","data":[{"p1":{"x":261.0333333333333,"y":170.40000000000003},"p2":{"x":321.4935689290364,"y":170.40000000000003},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da07343381308112318","data":[{"p1":{"x":261.0333333333333,"y":170.40000000000003},"p2":{"x":261.0333333333333,"y":229.5},"cp":{"dx":-10.033333333333331,"dy":25.09999999999998},"cp2":{"dx":-9.033333333333331,"dy":-18}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp9282897635669054","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":185},"p2":{"x":321.4935689290364,"y":214.09999084472645}}},{"id":"dp393874727676933","type":"rectangle","data":{"p1":{"x":321.4935689290364,"y":184.89999694824218},"p2":{"x":381.95380452473955,"y":213.99998779296862}}},{"id":"dp6993211133634349","type":"rectangle","data":{"p1":{"x":261.0333333333333,"y":266},"p2":{"x":321.4935689290364,"y":323}}},{"id":"dp012266046773700356","type":"rectangle","data":{"p1":{"x":321.3666666666667,"y":266},"p2":{"x":381.8269022623698,"y":323}}},{"id":"dp7393571113031379","type":"rectangle","data":{"p1":{"x":410.3666666666667,"y":266.33333333333337},"p2":{"x":470.8269022623698,"y":323.33333333333337}}},{"id":"dp1046271665702041","type":"rectangle","data":{"p1":{"x":470.70000000000005,"y":266.33333333333337},"p2":{"x":531.1602355957032,"y":323.33333333333337}}},{"id":"da627640078975749","data":[{"p1":{"x":321.3666666666666,"y":169.73333333333335},"p2":{"x":381.82690226236974,"y":169.73333333333335},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da2688917890203353","data":[{"p1":{"x":471.69999999999993,"y":169.73333333333335},"p2":{"x":532.160235595703,"y":169.73333333333335},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da979546034731009","data":[{"p1":{"x":411.03333333333325,"y":169.73333333333335},"p2":{"x":471.49356892903637,"y":169.73333333333335},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp8781662679227786","type":"rectangle","data":{"p1":{"x":410.7,"y":170},"p2":{"x":471.1602355957031,"y":227}}},{"id":"dp9634528922989665","type":"rectangle","data":{"p1":{"x":471.03333333333336,"y":170},"p2":{"x":531.4935689290364,"y":227}}},{"id":"da5810777676545826","data":[{"p1":{"x":531.4935689290364,"y":170},"p2":{"x":531.4935689290364,"y":227},"cp":{"dx":5.839764404296943,"dy":12},"cp2":{"dx":6.839764404296943,"dy":-14}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp5557708921089375","type":"down-arrow","data":{"p1":{"x":350.66666666666663,"y":64.83333333333331},"p2":{"x":373.5237833658854,"y":85.69047292073566},"rotation":269.56}},{"id":"dp4455056475410022","type":"rectangle","data":{"p1":{"x":407.0333333333333,"y":47.30000000000001},"p2":{"x":467.4935689290364,"y":61.60000000000002}}},{"id":"dp8444377655311619","type":"rectangle","data":{"p1":{"x":467.4935689290364,"y":47.30000000000001},"p2":{"x":527.9538045247396,"y":61.60000000000002}}},{"id":"dp3004786850902146","type":"rectangle","data":{"p1":{"x":407.0333333333333,"y":61.70000000000002},"p2":{"x":467.4935689290364,"y":76}}},{"id":"dp7381547876698642","type":"rectangle","data":{"p1":{"x":467.4935689290364,"y":61.70000000000002},"p2":{"x":527.9538045247396,"y":76}}},{"id":"dp07034288444646442","type":"rectangle","data":{"p1":{"x":407.0333333333333,"y":76},"p2":{"x":467.4935689290364,"y":90.30000000000001}}},{"id":"dp8210299596414079","type":"rectangle","data":{"p1":{"x":467.4935689290364,"y":76},"p2":{"x":527.9538045247396,"y":90.30000000000001}}},{"id":"dp9845084232040859","type":"rectangle","data":{"p1":{"x":407.0333333333333,"y":90.30000000000001},"p2":{"x":467.4935689290364,"y":106.5}},"style":{"fillColor":[218,216,216,0.6]}},{"id":"dp001261613544584872","type":"rectangle","data":{"p1":{"x":467.4935689290364,"y":90.30000000000001},"p2":{"x":527.9538045247396,"y":106.5}},"style":{"fillColor":[218,216,216,0.6]}},{"id":"da3986223462678937","data":[{"p1":{"x":407.0333333333333,"y":47.400000000000034},"p2":{"x":407.0333333333333,"y":61.70000000000002},"cp":{"dx":-4.166666666666664,"dy":5.833333333333336},"cp2":{"dx":-4.166666666666664,"dy":-6.799999999999997}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da1742461075880668","data":[{"p1":{"x":407.0333333333333,"y":47.400000000000034},"p2":{"x":467.4935689290364,"y":47.400000000000034},"cp":{"dx":13.833333333333329,"dy":-6.833333333333336},"cp2":{"dx":-15.293568929036454,"dy":-6.166666666666664}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da7421169241061067","data":[{"p1":{"x":407.0333333333333,"y":47.400000000000034},"p2":{"x":407.0333333333333,"y":106.5},"cp":{"dx":-10.033333333333331,"dy":25.09999999999998},"cp2":{"dx":-9.033333333333331,"dy":-18}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"}],"settings":{"grid":true,"gridSize":15,"diagramHeight":366.5}}]},{"id":"n0.5759487568923527","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":605,"sizeUnit":"px"}},"___version":2,"version":2,"av":1873,"delayRenderCache":{"av":1873,"map":{}}}

==> codes/docs/f8e793ed-042b-479e-9864-12645cf0d952 <==
{"id":"r0.4546527132442463","lines":[{"id":"n0.8764537390235608","blocks":[]},{"id":"n0.6785216271931982","blocks":[],"style":null},{"id":"n0.4573752054968587","blocks":[{"id":"n0.08615445619643625","text":"\\diagram","type":"composite","elements":{"de4056548892044547":{"id":"de4056548892044547","lines":[{"id":"n0.285263129718887","blocks":[{"id":"n0.8825849111109034","text":"1"}]}],"shape":{"data":{"p":{"x":32.19999999999999,"y":41.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de9172713841506903":{"id":"de9172713841506903","lines":[{"blocks":[{"id":"n0.8675176194344503","text":"2"}],"id":"n0.7613085187991293"}],"shape":{"data":{"p":{"x":52.19999999999999,"y":41.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de7611260175521506":{"id":"de7611260175521506","lines":[{"blocks":[{"id":"n0.07993386338898079","text":"3"}],"id":"n0.6774051432942736"}],"shape":{"data":{"p":{"x":72.19999999999999,"y":41.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de12079537535100981":{"id":"de12079537535100981","lines":[{"blocks":[{"id":"n0.2809150270011189","text":"4"}],"id":"n0.2891329786849286"}],"shape":{"data":{"p":{"x":92.19999999999999,"y":41.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de39648771184991327":{"id":"de39648771184991327","lines":[{"blocks":[{"id":"n0.4385326956920623","text":"5"}],"id":"n0.807902153580585"}],"shape":{"data":{"p":{"x":32.19999999999999,"y":61.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de6717583570042043":{"id":"de6717583570042043","lines":[{"blocks":[{"id":"n0.7395023435617096","text":"6"}],"id":"n0.7326677637121413"}],"shape":{"data":{"p":{"x":52.19999999999999,"y":61.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de7178146213895578":{"id":"de7178146213895578","lines":[{"blocks":[{"id":"n0.9181141987119545","text":"7"}],"id":"n0.4130871974140582"}],"shape":{"data":{"p":{"x":72.19999999999999,"y":61.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de35483280146710605":{"id":"de35483280146710605","lines":[{"blocks":[{"id":"n0.31157982794723105","text":"8"}],"id":"n0.2867824964133765"}],"shape":{"data":{"p":{"x":91.19999999999999,"y":61.40000000000001}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de41194111053158555":{"id":"de41194111053158555","lines":[{"blocks":[{"id":"n0.5523163208262845","text":"9"}],"id":"n0.5558762066293799"}],"shape":{"data":{"p":{"x":32.19999999999999,"y":81.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de45197794956127435":{"id":"de45197794956127435","lines":[{"blocks":[{"text":"10","id":"n0.0075773865950350405"}],"id":"n0.9429122800347995"}],"shape":{"data":{"p":{"x":49.19999999999999,"y":81.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de37709408732390304":{"id":"de37709408732390304","lines":[{"blocks":[{"text":"11","id":"n0.6892053191506837"}],"id":"n0.8189243751846216"}],"shape":{"data":{"p":{"x":69.19999999999999,"y":81.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de09747410369521092":{"id":"de09747410369521092","lines":[{"blocks":[{"text":"12","id":"n0.8536797441778674"}],"id":"n0.8015140025523129"}],"shape":{"data":{"p":{"x":88.19999999999999,"y":81.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de46670207273309994":{"id":"de46670207273309994","lines":[{"blocks":[{"text":"13","id":"n0.1180236755542361"}],"id":"n0.045514483427155916"}],"shape":{"data":{"p":{"x":29.19999999999999,"y":101.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de9921575259177471":{"id":"de9921575259177471","lines":[{"blocks":[{"text":"14","id":"n0.78531313975361"}],"id":"n0.9954368480390412"}],"shape":{"data":{"p":{"x":49.19999999999999,"y":101.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de3223092369832916":{"id":"de3223092369832916","lines":[{"blocks":[{"text":"15","id":"n0.0011577865029761547"}],"id":"n0.7388624268232507"}],"shape":{"data":{"p":{"x":69.19999999999999,"y":101.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de6717644950918429":{"id":"de6717644950918429","lines":[{"blocks":[{"text":"16","id":"n0.8104064995921232"}],"id":"n0.022002872052507616"}],"shape":{"data":{"p":{"x":89.19999999999999,"y":101.4}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de6905528661217077":{"id":"de6905528661217077","lines":[{"blocks":[{"text":"1","id":"n0.5629252222828578"}],"id":"n0.6933719008671633"}],"shape":{"data":{"p":{"x":146.5999999999999,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de8016560643997448":{"id":"de8016560643997448","lines":[{"blocks":[{"text":"2","id":"n0.952870109330145"}],"id":"n0.18909316604515714"}],"shape":{"data":{"p":{"x":166.5999999999999,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de9685059236389413":{"id":"de9685059236389413","lines":[{"blocks":[{"text":"3","id":"n0.3882891688875374"}],"id":"n0.38890840881716104"}],"shape":{"data":{"p":{"x":186.5999999999999,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de09149242922108414":{"id":"de09149242922108414","lines":[{"blocks":[{"id":"n0.46446945885495117","text":"14"}],"id":"n0.012701020279575426"}],"shape":{"data":{"p":{"x":263.5999999999999,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de908878586493366":{"id":"de908878586493366","lines":[{"blocks":[{"id":"n0.7101638613354657","text":"15"}],"id":"n0.8598793846122406"}],"shape":{"data":{"p":{"x":282.5999999999999,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de6941666773941773":{"id":"de6941666773941773","lines":[{"blocks":[{"text":"16","id":"n0.3284144982074957"}],"id":"n0.475209172845408"}],"shape":{"data":{"p":{"x":303.26666666666654,"y":71.06666666666669}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true},"de8047573819374771":{"id":"de8047573819374771","lines":[{"id":"n0.8214675561482137","blocks":[{"id":"n0.5155518165487207","text":"⋯"}]}],"shape":{"data":{"p":{"x":216.26666666666657,"y":69.06666666666669}},"anchor":"left-top"},"isMathDisplayMode":true},"de32689070498682793":{"id":"de32689070498682793","lines":[{"id":"n0.017855417729418344","blocks":[{"id":"n0.6322877604755928","text":"(a) row-wise packing"}]}],"shape":{"data":{"p":{"x":16.799999999999983,"y":12.400000000000013}},"anchor":"left-top"},"isTextMode":true},"de5471088034433311":{"id":"de5471088034433311","lines":[{"blocks":[{"text":"(b) block-wise matrix multiplication","id":"n0.039100575532635906"}],"id":"n0.8090673465207838"}],"shape":{"data":{"p":{"x":23.19999999999996,"y":139.8}},"anchor":"left-top"},"isTextMode":true},"de3611704217920588":{"id":"de3611704217920588","lines":[{"id":"n0.3036490116619446","blocks":[{"id":"n0.3243565417994074","text":"768"}]}],"shape":{"data":{"p":{"x":83.33333333333333,"y":200.6666641235352}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de503328275026236":{"id":"de503328275026236","lines":[{"blocks":[{"text":"768","id":"n0.09379098366036054"}],"id":"n0.0035605978546555672"}],"shape":{"data":{"p":{"x":227,"y":162.33333079020187}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de8591881421204302":{"id":"de8591881421204302","lines":[{"blocks":[{"text":"768","id":"n0.3645025184821937"}],"id":"n0.013209499274538183"}],"shape":{"data":{"p":{"x":320.0316451477803,"y":224.0739028695621},"rotation":89.33},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de43433377075030877":{"id":"de43433377075030877","lines":[{"blocks":[{"text":"128","id":"n0.7713929139302602"}],"id":"n0.07910103266017399"}],"shape":{"data":{"p":{"x":9.000000000000014,"y":229.3333307902019}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de8293066332484131":{"id":"de8293066332484131","lines":[{"blocks":[{"text":"768","id":"n0.9730620275727266"}],"id":"n0.10624086693107992"}],"shape":{"data":{"p":{"x":416.13333333333327,"y":200.6666641235352}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de8256814832972699":{"id":"de8256814832972699","lines":[{"blocks":[{"text":"128","id":"n0.8539694811729623"}],"id":"n0.2998766365561809"}],"shape":{"data":{"p":{"x":341.79999999999995,"y":229.3333307902019}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de24786466894276593":{"id":"de24786466894276593","lines":[{"blocks":[{"text":"128","id":"n0.39756809387851644"}],"id":"n0.8195174434065993"}],"shape":{"data":{"p":{"x":371.1333333333333,"y":255.99999745686853}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de9410444226791932":{"id":"de9410444226791932","lines":[{"blocks":[{"text":"⋯","id":"n0.826552621653516"}],"id":"n0.901586746139591"}],"shape":{"data":{"p":{"x":411.5999999999999,"y":224.73333333333335}},"anchor":"left-top"},"isMathDisplayMode":true},"de7605250251713673":{"id":"de7605250251713673","lines":[{"blocks":[{"text":"256","id":"n0.033668612240508766"}],"id":"n0.5209391761893367"}],"shape":{"data":{"p":{"x":42.333333333333314,"y":257.9999974568686}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de7943977454177453":{"id":"de7943977454177453","lines":[{"blocks":[{"text":"256","id":"n0.0145900025502963"}],"id":"n0.502611183127043"}],"shape":{"data":{"p":{"x":158.90469200698908,"y":211.88355922753217},"rotation":269.66},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de16887956001124338":{"id":"de16887956001124338","lines":[{"blocks":[{"text":"⋯","id":"n0.023627952446888312"}],"id":"n0.2526387922117532"}],"shape":{"data":{"p":{"x":222.26666666666654,"y":189.73333333333335}},"anchor":"left-top"},"isMathDisplayMode":true},"de29859351159712944":{"id":"de29859351159712944","lines":[{"blocks":[{"text":"⋯","id":"n0.49663265765443465"}],"id":"n0.8471429810409936"}],"shape":{"data":{"p":{"x":223.26666666666654,"y":230.73333333333335}},"anchor":"left-top"},"isMathDisplayMode":true},"de6749186196653831":{"id":"de6749186196653831","lines":[{"blocks":[{"text":"⋯","id":"n0.6250526728366532"}],"id":"n0.7175637403389514"}],"shape":{"data":{"p":{"x":222.93333333333322,"y":270.73333333333335}},"anchor":"left-top"},"isMathDisplayMode":true},"de18380788843170404":{"id":"de18380788843170404","lines":[{"id":"n0.46482837614020256","blocks":[{"id":"n0.6331446469397222","text":"A"}]}],"shape":{"data":{"p":{"x":45.000000000000014,"y":226}},"anchor":"left-top"},"isMathDisplayMode":true},"de37717992633978814":{"id":"de37717992633978814","lines":[{"blocks":[{"id":"n0.36260019361852747","text":"B"}],"id":"n0.11105144955513202"}],"shape":{"data":{"p":{"x":86.00000000000001,"y":225.33333333333331}},"anchor":"left-top"},"isMathDisplayMode":true},"de6768600457471776":{"id":"de6768600457471776","lines":[{"blocks":[{"id":"n0.1125560410038755","text":"C"}],"id":"n0.20351628390158183"}],"shape":{"data":{"p":{"x":124.33333333333334,"y":225.33333333333331}},"anchor":"left-top"},"isMathDisplayMode":true},"de08707254698976641":{"id":"de08707254698976641","lines":[{"blocks":[{"id":"n0.41166821826341793","text":"W"},{"id":"n0.8677407721091088","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9276361649115874","lines":[{"id":"n0.4968846200174475","blocks":[{"id":"n0.0880480176063545","text":" "}]}]}}},{"id":"n0.47121298565204905","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.11917045706185037","lines":[{"id":"n0.17001000682179757","blocks":[{"id":"n0.40642078170010154","text":"11"}]}]}}}],"id":"n0.3660656085056855"}],"shape":{"data":{"p":{"x":177.33333333333334,"y":190.66666666666669}},"anchor":"left-top"},"isMathDisplayMode":true},"de6124082032209854":{"id":"de6124082032209854","lines":[{"blocks":[{"text":"W","id":"n0.7257515542806947"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":" ","id":"n0.5132524627398989"}],"id":"n0.9139980666561269"}],"id":"n0.08660119618444706"}},"id":"n0.3241854445516248"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"21","id":"n0.5989535332296549"}],"id":"n0.17844744157724013"}],"id":"n0.8718266989088559"}},"id":"n0.5020880732880397"}],"id":"n0.2739107107816139"}],"shape":{"data":{"p":{"x":177.33333333333334,"y":230.66666666666669}},"anchor":"left-top"},"isMathDisplayMode":true},"de8694197177827545":{"id":"de8694197177827545","lines":[{"blocks":[{"text":"W","id":"n0.5563145834525469"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":" ","id":"n0.39163299150544906"}],"id":"n0.057609557403761835"}],"id":"n0.9250809579086674"}},"id":"n0.5531837557376427"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"31","id":"n0.6647956708276965"}],"id":"n0.841060825474357"}],"id":"n0.6806474715724036"}},"id":"n0.3305164982655935"}],"id":"n0.7231660336852714"}],"shape":{"data":{"p":{"x":177.66666666666669,"y":267.66666666666674}},"anchor":"left-top"},"isMathDisplayMode":true},"de017436197889418414":{"id":"de017436197889418414","lines":[{"blocks":[{"text":"W","id":"n0.2903849747594782"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":" ","id":"n0.6675268598748494"}],"id":"n0.17848038796847687"}],"id":"n0.5861502966697558"}},"id":"n0.17300114972606884"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"16","id":"n0.9933163253384785"}],"id":"n0.25288774491034527"}],"id":"n0.6953151286375718"}},"id":"n0.6291935178697252"}],"id":"n0.7841431227984839"}],"shape":{"data":{"p":{"x":266.66666666666674,"y":190.66666666666666}},"anchor":"left-top"},"isMathDisplayMode":true},"de7124294778223659":{"id":"de7124294778223659","lines":[{"blocks":[{"text":"128","id":"n0.9759955475855586"}],"id":"n0.8213045289252858"}],"shape":{"data":{"p":{"x":184,"y":305.99999745686864}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true},"de21910075667859874":{"id":"de21910075667859874","lines":[{"blocks":[{"text":"W","id":"n0.5414137502596108"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":" ","id":"n0.12800189399310224"}],"id":"n0.21037791865979805"}],"id":"n0.36528411908625946"}},"id":"n0.7809700906882722"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"26","id":"n0.3272946158280168"}],"id":"n0.5147251549930643"}],"id":"n0.7427243507405987"}},"id":"n0.31837119020804194"}],"id":"n0.20967634196941076"}],"shape":{"data":{"p":{"x":267,"y":229.99999999999997}},"anchor":"left-top"},"isMathDisplayMode":true},"de7642026354332134":{"id":"de7642026354332134","lines":[{"blocks":[{"text":"W","id":"n0.24735130886525236"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":" ","id":"n0.8763400609421124"}],"id":"n0.1458724114036587"}],"id":"n0.41342624129556316"}},"id":"n0.8818698758630568"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"36","id":"n0.13993292270455382"}],"id":"n0.7908254267954755"}],"id":"n0.4238909076460169"}},"id":"n0.6705202410067461"}],"id":"n0.24750166629643267"}],"shape":{"data":{"p":{"x":266.6666666666667,"y":268.3333333333334}},"anchor":"left-top"},"isMathDisplayMode":true},"de5064798759229545":{"id":"de5064798759229545","lines":[{"blocks":[{"id":"n0.8509312443998243","text":"res"},{"id":"n0.6683824741879731","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.42172228901585807","lines":[{"id":"n0.24352884233195016","blocks":[{"id":"n0.881859252308328","text":"1"}]}]}}}],"id":"n0.7576197355503906"}],"shape":{"data":{"p":{"x":368,"y":225}},"anchor":"left-top"},"isMathDisplayMode":true},"de04419183111598257":{"id":"de04419183111598257","lines":[{"blocks":[{"text":"res","id":"n0.016627834393648122"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2704794729319868","text":"6"}],"id":"n0.6817873144262137"}],"id":"n0.7841539692726676"}},"id":"n0.6851797567660396"}],"id":"n0.3379815805890889"}],"shape":{"data":{"p":{"x":457.33333333333337,"y":225}},"anchor":"left-top"},"isMathDisplayMode":true},"de4267646936378482":{"id":"de4267646936378482","lines":[{"blocks":[{"text":"res","id":"n0.4452417698024187"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.608363483659659"}],"id":"n0.33882418380837076"}],"id":"n0.5440781443763358"}},"id":"n0.012763735823564382"},{"id":"n0.3868461306419937","text":"= A×W"},{"id":"n0.587423946715826","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1952111936046117","lines":[{"id":"n0.9737604105907374","blocks":[{"id":"n0.4882616245513929","text":"11"}]}]}}},{"id":"n0.4399238937594703","text":"+ B×W"},{"id":"n0.4913118014432032","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.31536856622567666","lines":[{"id":"n0.8856111540410263","blocks":[{"id":"n0.7088559136993748","text":"21"}]}]}}},{"id":"n0.14465069868345082","text":" + C×W"},{"id":"n0.7157456746390403","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.723280697494572","lines":[{"id":"n0.10792649802694654","blocks":[{"id":"n0.8606773372941987","text":"31"}]}]}}}],"id":"n0.8404223497981655"}],"shape":{"data":{"p":{"x":340.99999999999994,"y":279.6666666666667}},"anchor":"left-top"},"isMathDisplayMode":true},"de28743590293819854":{"id":"de28743590293819854","lines":[{"blocks":[{"text":"res","id":"n0.7244768959279095"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9547511516740286","text":"6"}],"id":"n0.1394302819248252"}],"id":"n0.43934966540813036"}},"id":"n0.44814484171366575"},{"text":"= A×W","id":"n0.8562300284380504"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"16","id":"n0.2862873200838436"}],"id":"n0.17270256067644607"}],"id":"n0.9016338007883722"}},"id":"n0.9130302966595181"},{"text":"+ B×W","id":"n0.7292538323632043"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"26","id":"n0.020526505843193155"}],"id":"n0.8271377311020642"}],"id":"n0.6888274432437844"}},"id":"n0.375345373109101"},{"text":" + C×W","id":"n0.03188345700469308"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"36","id":"n0.1675927979210874"}],"id":"n0.7281260643350669"}],"id":"n0.6730158612111321"}},"id":"n0.20631524723798145"}],"id":"n0.3756745320857422"}],"shape":{"data":{"p":{"x":341.6666666666666,"y":322.33333333333337}},"anchor":"left-top"},"isMathDisplayMode":true},"de9344162839617973":{"id":"de9344162839617973","lines":[{"id":"n0.16660334605153126","blocks":[{"id":"n0.25736015939684953","text":"×"}]}],"shape":{"data":{"p":{"x":155.75998535156248,"y":225.43999938964845}},"anchor":"left-top"},"isMathDisplayMode":true},"de7284721213145531":{"id":"de7284721213145531","lines":[{"blocks":[{"id":"n0.4874547063433965","text":"="}],"id":"n0.13529522176166386"}],"shape":{"data":{"p":{"x":321.09331868489585,"y":224.10666605631513}},"anchor":"left-top"},"isMathDisplayMode":true},"de9883508887020607":{"id":"de9883508887020607","lines":[{"blocks":[{"text":"⋯","id":"n0.8817793528106945"}],"id":"n0.21584926999771614"}],"shape":{"data":{"p":{"x":511.3814428570367,"y":296.5321906284913},"rotation":89.82},"anchor":"left-top"},"isMathDisplayMode":true},"de5915525666708756":{"id":"de5915525666708756","lines":[{"blocks":[{"text":"128","id":"n0.6203637907625115"}],"id":"n0.6187206970945527"}],"shape":{"data":{"p":{"x":460.46666666666664,"y":255.33333079020184}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true}},"connections":[],"intersections":{"id":"di32816999271940284","items":[],"style":{}},"shapes":[{"id":"dp8887336422334198","type":"square","data":{"p1":{"x":29.19999999999999,"y":41.40000000000001},"p2":{"x":49.19999999999999,"y":61.40000000000001}}},{"id":"dp8102807124985265","type":"square","data":{"p1":{"x":49.19999999999999,"y":41.40000000000001},"p2":{"x":69.19999999999999,"y":61.40000000000001}}},{"id":"dp4893595360558587","type":"square","data":{"p1":{"x":49.19999999999999,"y":61.40000000000001},"p2":{"x":69.19999999999999,"y":81.4}}},{"id":"dp6458624710781111","type":"square","data":{"p1":{"x":29.19999999999999,"y":61.40000000000001},"p2":{"x":49.19999999999999,"y":81.4}}},{"id":"dp47086007921406225","type":"square","data":{"p1":{"x":69.19999999999999,"y":41.40000000000001},"p2":{"x":89.19999999999999,"y":61.40000000000001}}},{"id":"dp1057589979866127","type":"square","data":{"p1":{"x":89.19999999999999,"y":41.40000000000001},"p2":{"x":109.19999999999999,"y":61.40000000000001}}},{"id":"dp6168662302435235","type":"square","data":{"p1":{"x":89.19999999999999,"y":61.40000000000001},"p2":{"x":109.19999999999999,"y":81.4}}},{"id":"dp13862915594021086","type":"square","data":{"p1":{"x":69.19999999999999,"y":61.40000000000001},"p2":{"x":89.19999999999999,"y":81.4}}},{"id":"dp6342553034357066","type":"square","data":{"p1":{"x":29.19999999999999,"y":81.4},"p2":{"x":49.19999999999999,"y":101.4}}},{"id":"dp18483789937900896","type":"square","data":{"p1":{"x":49.19999999999999,"y":81.4},"p2":{"x":69.19999999999999,"y":101.4}}},{"id":"dp3797405866097008","type":"square","data":{"p1":{"x":49.19999999999999,"y":101.4},"p2":{"x":69.19999999999999,"y":121.4}}},{"id":"dp9847358104028017","type":"square","data":{"p1":{"x":29.19999999999999,"y":101.4},"p2":{"x":49.19999999999999,"y":121.4}}},{"id":"dp8481176217309965","type":"square","data":{"p1":{"x":69.19999999999999,"y":81.4},"p2":{"x":89.19999999999999,"y":101.4}}},{"id":"dp6613125262125283","type":"square","data":{"p1":{"x":89.19999999999999,"y":81.4},"p2":{"x":109.19999999999999,"y":101.4}}},{"id":"dp6805788122286043","type":"square","data":{"p1":{"x":89.19999999999999,"y":101.4},"p2":{"x":109.19999999999999,"y":121.4}}},{"id":"dp8213431635852444","type":"square","data":{"p1":{"x":69.19999999999999,"y":101.4},"p2":{"x":89.19999999999999,"y":121.4}}},{"id":"dp16497673595700202","type":"square","data":{"p1":{"x":143.5999999999999,"y":71.06666666666669},"p2":{"x":163.5999999999999,"y":91.06666666666669}}},{"id":"dp8295520587876786","type":"square","data":{"p1":{"x":163.5999999999999,"y":71.06666666666669},"p2":{"x":183.5999999999999,"y":91.06666666666669}}},{"id":"dp9898086800277017","type":"square","data":{"p1":{"x":183.5999999999999,"y":71.06666666666669},"p2":{"x":203.5999999999999,"y":91.06666666666669}}},{"id":"dp07067083930593299","type":"square","data":{"p1":{"x":263.5999999999999,"y":71.06666666666669},"p2":{"x":283.5999999999999,"y":91.06666666666669}}},{"id":"dp4773143444884618","type":"square","data":{"p1":{"x":283.5999999999999,"y":71.06666666666669},"p2":{"x":303.5999999999999,"y":91.06666666666669}}},{"id":"dp5039929773349914","type":"square","data":{"p1":{"x":303.26666666666654,"y":71.06666666666669},"p2":{"x":323.26666666666654,"y":91.06666666666669}}},{"id":"dp588530209940924","type":"rectangle","data":{"p1":{"x":203.21905924479148,"y":71.06666666666669},"p2":{"x":263.5999999999999,"y":91.20000000000002}}},{"id":"da18778411973516929","data":[{"x":39.19999999999999,"y":51.40000000000001},{"x":87,"y":51.40000000000001},{"x":99.19999999999999,"y":51.40000000000001}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"da3574442515134162","data":[{"x":99.19999999999999,"y":51.40000000000001},{"x":99.19999999999999,"y":51.40000000000001},{"x":39.19999999999999,"y":71.4}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"da33477504659417456","data":[{"x":39.999999999999986,"y":71.4},{"x":87.8,"y":71.4},{"x":99.99999999999999,"y":71.4}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"da8427884052445369","data":[{"x":99.99999999999999,"y":71.4},{"x":99.99999999999999,"y":71.4},{"x":39.999999999999986,"y":91.4}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"da2891678086257845","data":[{"x":39.999999999999986,"y":91.4},{"x":87.8,"y":91.4},{"x":99.99999999999999,"y":91.4}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"da18425598054553882","data":[{"x":99.99999999999999,"y":91.4},{"x":99.99999999999999,"y":91.4},{"x":39.999999999999986,"y":111.4}],"head":">","tail":"no","shaft":"-","mVer":1,"headScale":1,"style":{"thickness":2,"fillColor":[241,181,255,1],"strokeColor":[14,14,14,0.58]}},{"id":"dp26826872694244264","type":"right-arrow","data":{"p1":{"x":122.39999999999995,"y":73.55999755859375},"p2":{"x":137.59999999999997,"y":87.6}}},{"id":"dp7144729072843101","type":"rectangle","data":{"p1":{"x":35.2,"y":223.43999938964845},"p2":{"x":74.7199951171875,"y":252.8}},"style":{"fillColor":[235,244,252,0.83]}},{"id":"dp9413200931218284","type":"rectangle","data":{"p1":{"x":74.7199951171875,"y":223.43999938964845},"p2":{"x":114.23999023437499,"y":252.8}},"style":{"fillColor":[220,248,187,0.6]}},{"id":"dp30498394157359954","type":"rectangle","data":{"p1":{"x":114.23999023437499,"y":223.43999938964845},"p2":{"x":153.75998535156248,"y":252.8}},"style":{"fillColor":[248,199,199,0.6]}},{"id":"dp2617893403763447","type":"rectangle","data":{"p1":{"x":175.8855074198064,"y":188.32001932055874},"p2":{"x":215.40550253699385,"y":217.68001993091028},"rotation":89.95},"style":{"fillColor":[214,211,211,0.6]}},{"id":"dp3092364012238693","type":"rectangle","data":{"p1":{"x":175.9199951171875,"y":227.83999938964848},"p2":{"x":215.43999023437493,"y":257.20000000000005},"rotation":89.95},"style":{"fillColor":[146,146,146,0.6]}},{"id":"dp27564242982449527","type":"rectangle","data":{"p1":{"x":175.95448281456856,"y":267.35997945873817},"p2":{"x":215.47447793175598,"y":296.7199800690897},"rotation":89.95},"style":{"fillColor":[46,45,45,0.6]}},{"id":"dp5177611953754366","type":"rectangle","data":{"p1":{"x":220.60345308715452,"y":172.92303345698807},"p2":{"x":260.1234482043418,"y":232.99895823600653},"rotation":89.95}},{"id":"dp027639785618825297","type":"rectangle","data":{"p1":{"x":220.62034205684606,"y":212.46062761825942},"p2":{"x":260.14033717403345,"y":272.5013549284967},"rotation":89.95}},{"id":"dp6019417166244394","type":"rectangle","data":{"p1":{"x":220.63766735862913,"y":251.9977850665014},"p2":{"x":260.15766247581644,"y":312.0041875724728},"rotation":89.95}},{"id":"dp9485138846534087","type":"rectangle","data":{"p1":{"x":265.27215294825845,"y":188.26877645915891},"p2":{"x":304.7921480654459,"y":217.62877706951045},"rotation":89.95},"style":{"fillColor":[202,201,214,0.6]}},{"id":"dp584574229183499","type":"rectangle","data":{"p1":{"x":265.3066406456395,"y":227.78875652824854},"p2":{"x":304.82663576282687,"y":257.1487571386001},"rotation":89.95},"style":{"fillColor":[140,144,153,0.6]}},{"id":"dp8360210291324157","type":"rectangle","data":{"p1":{"x":265.3411283430204,"y":267.3087365973382},"p2":{"x":304.86112346020786,"y":296.66873720768973},"rotation":89.95},"style":{"fillColor":[70,70,77,0.6]}},{"id":"da8079063536264146","data":[{"p1":{"x":35.2,"y":223.43999938964845},"p2":{"x":95.06676012184985,"y":215.7347742794064},"cp":{"dx":12.292038871886966,"dy":-5.063784433076677},"cp2":{"dx":-23.701593788436796,"dy":0.031106577845633865}},{"p1":{"x":95.06676012184985,"y":215.7347742794064},"p2":{"x":98.39334920527125,"y":215.74737802539263},"cp":{"dx":1.1096410052150816,"dy":-0.001456321233831659},"cp2":{"dx":-1.107683048261535,"dy":-0.009863120806215875}},{"p1":{"x":98.39334920527125,"y":215.74737802539263},"p2":{"x":107.7862187825529,"y":215.96963651128252},"cp":{"dx":3.153046843911781,"dy":0.028075614209313926},"cp2":{"dx":-3.09959421443682,"dy":-0.12019593908070192}},{"p1":{"x":107.7862187825529,"y":215.96963651128252},"p2":{"x":153.75998535156248,"y":223.43999938964845},"cp":{"dx":18.97416700300893,"dy":0.7357794806102049},"cp2":{"dx":-9.548112358176525,"dy":-4.267224617432021}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da01120537655763254","data":[{"p1":{"x":181.13491602204562,"y":183.17597601443987},"p2":{"x":241.00167614389545,"y":175.4707509041978},"cp":{"dx":12.292038871886966,"dy":-5.063784433076677},"cp2":{"dx":-23.701593788436796,"dy":0.031106577845633865}},{"p1":{"x":241.00167614389545,"y":175.4707509041978},"p2":{"x":244.32826522731685,"y":175.48335465018405},"cp":{"dx":1.1096410052150816,"dy":-0.001456321233831659},"cp2":{"dx":-1.107683048261535,"dy":-0.009863120806215875}},{"p1":{"x":244.32826522731685,"y":175.48335465018405},"p2":{"x":253.72113480459848,"y":175.70561313607394},"cp":{"dx":3.153046843911781,"dy":0.028075614209313926},"cp2":{"dx":-3.09959421443682,"dy":-0.12019593908070192}},{"p1":{"x":253.72113480459848,"y":175.70561313607394},"p2":{"x":299.69490137360805,"y":183.17597601443987},"cp":{"dx":18.97416700300893,"dy":0.7357794806102049},"cp2":{"dx":-9.548112358176525,"dy":-4.267224617432021}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da06996406088607543","data":[{"p1":{"x":299.69490137360805,"y":183.17597601443987},"p2":{"x":299.798364465751,"y":301.7359162217089},"cp":{"dx":10.038436028735703,"dy":19.157357318893474},"cp2":{"dx":9.934972936592771,"dy":-18.402582888375605}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da805237134995469","data":[{"p1":{"x":35.2,"y":223.43999938964845},"p2":{"x":35.2,"y":252.8},"cp":{"dx":-4.7999959309895885,"dy":9.226667277018208},"cp2":{"dx":-4.466662597656253,"dy":-8.133333333333354}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp05358279247086073","type":"rectangle","data":{"p1":{"x":367.99999999999994,"y":223.43999938964845},"p2":{"x":398.60986328125,"y":252.8}},"style":{"fillColor":[243,224,252,0.6]}},{"id":"dp3415187045573935","type":"rectangle","data":{"p1":{"x":398.60986328125,"y":223.43999938964845},"p2":{"x":458.60986328125,"y":252.8}}},{"id":"dp3053252794556891","type":"rectangle","data":{"p1":{"x":458.60986328125,"y":223.43999938964845},"p2":{"x":486.55998535156243,"y":252.8}},"style":{"fillColor":[215,176,245,0.6]}},{"id":"da16409757140770798","data":[{"p1":{"x":367.99999999999994,"y":223.43999938964845},"p2":{"x":427.8667601218498,"y":215.7347742794064},"cp":{"dx":12.292038871886966,"dy":-5.063784433076677},"cp2":{"dx":-23.701593788436796,"dy":0.031106577845633865}},{"p1":{"x":427.8667601218498,"y":215.7347742794064},"p2":{"x":431.1933492052712,"y":215.74737802539263},"cp":{"dx":1.1096410052150816,"dy":-0.001456321233831659},"cp2":{"dx":-1.107683048261535,"dy":-0.009863120806215875}},{"p1":{"x":431.1933492052712,"y":215.74737802539263},"p2":{"x":440.5862187825528,"y":215.96963651128252},"cp":{"dx":3.153046843911781,"dy":0.028075614209313926},"cp2":{"dx":-3.09959421443682,"dy":-0.12019593908070192}},{"p1":{"x":440.5862187825528,"y":215.96963651128252},"p2":{"x":486.55998535156243,"y":223.43999938964845},"cp":{"dx":18.97416700300893,"dy":0.7357794806102049},"cp2":{"dx":-9.548112358176525,"dy":-4.267224617432021}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da3174872647167193","data":[{"p1":{"x":367.99999999999994,"y":223.43999938964845},"p2":{"x":367.99999999999994,"y":252.8},"cp":{"dx":-4.7999959309895885,"dy":9.226667277018208},"cp2":{"dx":-4.466662597656253,"dy":-8.133333333333354}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da46472241216062526","data":[{"p1":{"x":367.99999999999994,"y":252.8},"p2":{"x":398.60986328125,"y":252.8},"cp":{"dx":9.943196614583428,"dy":8.15075480143227},"cp2":{"dx":-9.666666666666629,"dy":7.484088134765585}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da619416697107392","data":[{"p1":{"x":35.2,"y":252.8},"p2":{"x":74.7199951171875,"y":252.8},"cp":{"dx":13.799999999999997,"dy":7.533333333333303},"cp2":{"dx":-13.719995117187494,"dy":7.866666666666674}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da6720492759531538","data":[{"p1":{"x":180.9482664142633,"y":183.2528403065396},"p2":{"x":180.98275411164434,"y":222.77282037562938},"cp":{"dx":-8.614933080929944,"dy":5.7471596934603895},"cp2":{"dx":-6.98275411164434,"dy":-6.439487042296065}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da04171923624713836","data":[{"p1":{"x":181.0517295064065,"y":301.8127805138088},"p2":{"x":210.41171893729916,"y":301.7871590831088},"cp":{"dx":8.662544582135155,"dy":5.425317630722475},"cp2":{"dx":-10.030778182090842,"dy":6.117605728089131}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da5146456410663116","data":[{"p1":{"x":457.33333333333326,"y":252.13333333333333},"p2":{"x":487.9431966145833,"y":252.13333333333333},"cp":{"dx":9.943196614583428,"dy":8.15075480143227},"cp2":{"dx":-9.666666666666629,"dy":7.484088134765585}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"}],"settings":{"grid":true,"diagramHeight":352.66666666666663}}]},{"id":"n0.4369273399181315","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1957,"delayRenderCache":{"av":1957,"map":{}}}

==> figures/GKTF_flow.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, scale = 0.75]
%uncomment if require: \path (0,199); %set diagram left start at 0, and has height of 199

%Rounded Rect [id:dp17239388731232408] 
\draw   (30.47,49.53) .. controls (30.47,45.23) and (33.95,41.75) .. (38.25,41.75) -- (73.39,41.75) .. controls (77.68,41.75) and (81.17,45.23) .. (81.17,49.53) -- (81.17,72.87) .. controls (81.17,77.17) and (77.68,80.65) .. (73.39,80.65) -- (38.25,80.65) .. controls (33.95,80.65) and (30.47,77.17) .. (30.47,72.87) -- cycle ;
%Rounded Rect [id:dp8321462215389779] 
\draw   (99.2,49.93) .. controls (99.2,45.63) and (102.68,42.15) .. (106.98,42.15) -- (148.62,42.15) .. controls (152.92,42.15) and (156.4,45.63) .. (156.4,49.93) -- (156.4,73.27) .. controls (156.4,77.57) and (152.92,81.05) .. (148.62,81.05) -- (106.98,81.05) .. controls (102.68,81.05) and (99.2,77.57) .. (99.2,73.27) -- cycle ;
%Rounded Rect [id:dp04331218543772297] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (182.8,50.13) .. controls (182.8,45.83) and (186.28,42.35) .. (190.58,42.35) -- (232.22,42.35) .. controls (236.52,42.35) and (240,45.83) .. (240,50.13) -- (240,73.47) .. controls (240,77.77) and (236.52,81.25) .. (232.22,81.25) -- (190.58,81.25) .. controls (186.28,81.25) and (182.8,77.77) .. (182.8,73.47) -- cycle ;
%Image [id:dp46764431784059735] 
\draw (169.13,44.95) node  {\includegraphics[width=17.8pt,height=18.55pt]{figures/lock.png}};
%Rounded Rect [id:dp30802804999068556] 
\draw   (30.8,99.53) .. controls (30.8,95.23) and (34.28,91.75) .. (38.58,91.75) -- (73.72,91.75) .. controls (78.02,91.75) and (81.5,95.23) .. (81.5,99.53) -- (81.5,122.87) .. controls (81.5,127.17) and (78.02,130.65) .. (73.72,130.65) -- (38.58,130.65) .. controls (34.28,130.65) and (30.8,127.17) .. (30.8,122.87) -- cycle ;
%Rounded Rect [id:dp4119095097252945] 
\draw   (99.53,99.93) .. controls (99.53,95.63) and (103.02,92.15) .. (107.31,92.15) -- (148.95,92.15) .. controls (153.25,92.15) and (156.73,95.63) .. (156.73,99.93) -- (156.73,123.27) .. controls (156.73,127.57) and (153.25,131.05) .. (148.95,131.05) -- (107.31,131.05) .. controls (103.02,131.05) and (99.53,127.57) .. (99.53,123.27) -- cycle ;
%Rounded Rect [id:dp6537819509218907] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (183.13,100.13) .. controls (183.13,95.83) and (186.62,92.35) .. (190.91,92.35) -- (232.55,92.35) .. controls (236.85,92.35) and (240.33,95.83) .. (240.33,100.13) -- (240.33,123.47) .. controls (240.33,127.77) and (236.85,131.25) .. (232.55,131.25) -- (190.91,131.25) .. controls (186.62,131.25) and (183.13,127.77) .. (183.13,123.47) -- cycle ;
%Flowchart: Multidocument [id:dp8633771479240973] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (315.68,38.67) -- (369.05,38.67) -- (369.05,66.88) .. controls (335.69,66.88) and (342.36,77.05) .. (315.68,70.47) -- cycle ; 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225  }  ,fill opacity=1 ] (309,42.94) -- (362.38,42.94) -- (362.38,71.15) .. controls (329.02,71.15) and (335.69,81.32) .. (309,74.74) -- cycle ; 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225  }  ,fill opacity=1 ] (302.33,47.22) -- (355.7,47.22) -- (355.7,75.42) .. controls (322.35,75.42) and (329.02,85.6) .. (302.33,79.02) -- cycle ;
%Flowchart: Multidocument [id:dp016896613618019973] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (412.77,29.33) -- (497.34,29.33) -- (497.34,67.79) .. controls (444.49,67.79) and (455.06,81.66) .. (412.77,72.68) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (402.2,35.16) -- (486.77,35.16) -- (486.77,73.62) .. controls (433.92,73.62) and (444.49,87.48) .. (402.2,78.51) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (391.63,40.99) -- (476.2,40.99) -- (476.2,79.44) .. controls (423.34,79.44) and (433.92,93.31) .. (391.63,84.34) -- cycle ;
%Image [id:dp48502379161272335] 
\draw (404.65,59.18) node  {\includegraphics[width=24.47pt,height=22.4pt]{figures/snow.png}};
%Flowchart: Multidocument [id:dp0659400597438593] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (363.1,134) -- (421,134) -- (421,162.17) .. controls (384.82,162.17) and (392.05,172.33) .. (363.1,165.76) -- cycle ; \draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (355.87,138.27) -- (413.76,138.27) -- (413.76,166.44) .. controls (377.58,166.44) and (384.82,176.6) .. (355.87,170.02) -- cycle ; \draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (348.63,142.54) -- (406.53,142.54) -- (406.53,170.71) .. controls (370.34,170.71) and (377.58,180.87) .. (348.63,174.29) -- cycle ;
%Straight Lines [id:da2756916523793138] 
\draw    (241,111.75) -- (289.75,111.75) ;
%Straight Lines [id:da9097862402599541] 
\draw    (289.75,111.75) -- (290,148.5) ;
%Straight Lines [id:da9231144380911036] 
\draw    (327,79) -- (327.25,102.75) ;
%Straight Lines [id:da4532131917741562] 
\draw    (327.25,102.75) -- (434.25,102.5) ;
%Straight Lines [id:da7227023217801751] 
\draw    (434,84.5) -- (434.25,102.5) ;
%Rounded Rect [id:dp9759151550655041] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (157.89,150.13) .. controls (157.89,145.83) and (161.37,142.35) .. (165.67,142.35) -- (218.55,142.35) .. controls (222.85,142.35) and (226.33,145.83) .. (226.33,150.13) -- (226.33,173.47) .. controls (226.33,177.77) and (222.85,181.25) .. (218.55,181.25) -- (165.67,181.25) .. controls (161.37,181.25) and (157.89,177.77) .. (157.89,173.47) -- cycle ;
%Rounded Rect [id:dp8665597765685331] 
\draw   (55.89,149.88) .. controls (55.89,145.58) and (59.37,142.1) .. (63.67,142.1) -- (116.55,142.1) .. controls (120.85,142.1) and (124.33,145.58) .. (124.33,149.88) -- (124.33,173.22) .. controls (124.33,177.52) and (120.85,181) .. (116.55,181) -- (63.67,181) .. controls (59.37,181) and (55.89,177.52) .. (55.89,173.22) -- cycle ;
%Image [id:dp2299970336373678] 
\draw (143.38,151.13) node  {\includegraphics[width=18.94pt,height=17.81pt]{figures/key.png}};
%Image [id:dp3912093589885002] 
\draw (540.9,96.18) node  {\includegraphics[width=24.47pt,height=22.4pt]{figures/snow.png}};
%Rounded Rect [id:dp6387708840441362] 
\draw  [fill={rgb, 255:red, 225; green, 225; blue, 225 }  ,fill opacity=1 ] (525.8,63.22) .. controls (525.8,60.93) and (527.65,59.08) .. (529.93,59.08) -- (551.28,59.08) .. controls (553.57,59.08) and (555.42,60.93) .. (555.42,63.22) -- (555.42,75.62) .. controls (555.42,77.9) and (553.57,79.75) .. (551.28,79.75) -- (529.93,79.75) .. controls (527.65,79.75) and (525.8,77.9) .. (525.8,75.62) -- cycle ;
%Rounded Rect [id:dp47030858483574844] 
\draw   (526.16,33.71) .. controls (526.16,31.45) and (527.99,29.62) .. (530.25,29.62) -- (551.07,29.62) .. controls (553.33,29.62) and (555.17,31.45) .. (555.17,33.71) -- (555.17,45.99) .. controls (555.17,48.25) and (553.33,50.08) .. (551.07,50.08) -- (530.25,50.08) .. controls (527.99,50.08) and (526.16,48.25) .. (526.16,45.99) -- cycle ;
%Straight Lines [id:da328149300120792] 
\draw    (165.21,14.96) -- (257.16,15.03) ;
%Straight Lines [id:da9178249438038648] 
\draw    (23.46,14.96) -- (115.41,15.03) ;
%Straight Lines [id:da28633893711232505] 
\draw    (423.46,15.34) -- (515.41,15.42) ;
%Straight Lines [id:da9141993194470628] 
\draw    (281.46,15.09) -- (373.41,15.17) ;
%Straight Lines [id:da713015238829519] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (268.75,5) -- (268.5,186.25) ;
%Straight Lines [id:da30857443268384355] 
\draw    (80.86,60) -- (95.52,60) ;
\draw [shift={(98.52,60)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5950041547572325] 
\draw    (156.52,60.67) -- (179.52,60.67) ;
\draw [shift={(182.52,60.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da509407416086282] 
\draw    (239.86,60.67) -- (298.52,60.67) ;
\draw [shift={(301.52,60.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da36211807065616264] 
\draw    (380.75,102.63) -- (380.85,135) ;
\draw [shift={(380.86,138)}, rotate = 269.83] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Image [id:dp5971926272510995] 
\draw (169.13,95.95) node  {\includegraphics[width=17.8pt,height=18.55pt]{figures/lock.png}};
%Straight Lines [id:da21896870625069864] 
\draw    (80.86,111) -- (95.52,111) ;
\draw [shift={(98.52,111)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da19747919700313066] 
\draw    (156.52,111.67) -- (179.52,111.67) ;
\draw [shift={(182.52,111.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7422209144128282] 
\draw    (290,148.5) -- (345.19,148.75) ;
\draw [shift={(348.19,148.76)}, rotate = 180.26] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3373856322036277] 
\draw    (230,162.08) -- (348.19,161.76) ;
\draw [shift={(227,162.08)}, rotate = 359.85] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da414905672735002] 
\draw    (127.86,161.41) -- (156.82,161.2) ;
\draw [shift={(124.86,161.43)}, rotate = 359.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (42,52) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{18.71pt}\setlength\topsep{0pt}
\begin{center}
Train\\data
\end{center}

\end{minipage}};
% Text Node
\draw (99.78,52) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{38.83pt}\setlength\topsep{0pt}
\begin{center}
Token\\Embedding
\end{center}

\end{minipage}};
% Text Node
\draw (159.27,64.32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\mathsf{Enc}$};
% Text Node
\draw (43,101) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{16.6pt}\setlength\topsep{0pt}
\begin{center}
Eval\\data
\end{center}

\end{minipage}};
% Text Node
\draw (100.36,101) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{38.83pt}\setlength\topsep{0pt}
\begin{center}
Token\\Embedding
\end{center}

\end{minipage}};
% Text Node
\draw (329, 63) node [anchor=center][inner sep=0.75pt]  [font=\scriptsize] [align=center] {
\scriptsize Fine-tuned\\
\scriptsize LoRA weight
};

% Text Node
\draw (412.33,45.73) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{43.58pt}\setlength\topsep{0pt}
\begin{center}
Pre-trained\\(frozen)\\LLM with GK
\end{center}

\end{minipage}};
% Text Node
\draw (354,146) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{32.48pt}\setlength\topsep{0pt}
\begin{center}
Inference
\end{center}

\end{minipage}};
% Text Node
\draw (183.78,52) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{38.83pt}\setlength\topsep{0pt}
\begin{center}
Token\\Embedding
\end{center}

\end{minipage}};
% Text Node
\draw (184.36,101) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{38.83pt}\setlength\topsep{0pt}
\begin{center}
Token\\Embedding
\end{center}

\end{minipage}};
% Text Node
\draw (159.36,152) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{44.77pt}\setlength\topsep{0pt}
\begin{center}
Classification\\score
\end{center}

\end{minipage}};
% Text Node
\draw (58.36,152) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{44.77pt}\setlength\topsep{0pt}
\begin{center}
Classification\\score
\end{center}

\end{minipage}};
% Text Node
\draw (131.75,166) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\mathsf{Dec}$};
% Text Node
\draw (558.75,33.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Plaintext};
% Text Node
\draw (558.5,62.25) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Ciphertext};
% Text Node
\draw (559.25,90.25) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Frozen weight};
% Text Node
\draw (118.75,7.62) node [anchor=north west][inner sep=0.75pt]   [align=left] {Client};
% Text Node
\draw (377,7.62) node [anchor=north west][inner sep=0.75pt]   [align=left] {Server};
% Text Node
\draw (159.27,115.32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\mathsf{Enc}$};


\end{tikzpicture}
